Parametric Session States Recover Retrieval Intent without Replaying History

Long-running assistants often interpret follow-up requests whose referents, constraints, and active goals were established many turns earlier. The central challenge is therefore not only context length, but retrieval intent: a current query such as ``use the previous configuration'' may omit the project, entity, and version terms needed to locate relevant evidence. Long-context models can recover those terms by replaying the interaction, but repeatedly pay the cost of processing history. Conventional retrieval-augmented generation (RAG) is cheaper, yet assumes an information-sufficient query; conversational rewriting either rereads the history or depends on an explicitly maintained textual memory. We introduce \emph{Parametric Session State} (\method{}), a reusable session-memory layer that remembers what to search for while keeping factual knowledge external.

==> ALGORITHM_TWO_STAGE_WRITER_20260905.tex <==
% Standalone replacement fragment; requires algorithm + algpseudocode + amsmath.
% Describes the selected retrieval_aligned configuration in the current code.
\begin{algorithm}[t]
\caption{Two-stage retrieval-supervised session-state compilation}
\label{alg:pss_two_stage_writer}
\begin{algorithmic}[1]
\Require Frozen base model $\theta$; ordered history $H_s$;
answer-free clues $(z_s^+,z_s^-)$; writer seed $\xi$
\Ensure BF16 session-specific LoRA state $\Delta_s$
\State Initialize rank-$32$ LoRA factors using $\xi$:
$A\sim\mathrm{KaimingUniform}$, $B=0$; freeze $\theta$
\State Split $H_s$ into ordered $128$-token chunks
$x_1,\ldots,x_M$, retaining chunks with at least two tokens
\State Initialize AdamW on $\Delta_s$ with learning rate $2\times10^{-5}$
\For{$t=1,\ldots,\max(16,M)$}
    \State $j\gets 1+((t-1)\bmod M)$
    \State $L\gets\mathcal L_{\mathrm{LM}}(x_j;\theta+\Delta_s)$
    \State Update $\Delta_s$ only; clip gradient norm to $1.0$
\EndFor
\State Discard the first optimizer and initialize a new AdamW
on $\Delta_s$ with learning rate $10^{-4}$
\State $p\gets$ fixed compact-search-clue readout instruction
\For{$t=1,\ldots,64$}
    \State $\ell^+\gets-\frac{1}{|z_s^+|}\log p_{\theta+\Delta_s}(z_s^+\mid p)$
    \State $\ell^-\gets-\frac{1}{|z_s^-|}\log p_{\theta+\Delta_s}(z_s^-\mid p)$
    \State $L\gets\ell^++\max(0,0.2+\ell^+-\ell^-)$
    \State Update $\Delta_s$ only; clip gradient norm to $1.0$
\EndFor
\State Verify finite factors; cast the state to BF16 and serialize it
with its session, seed, model, and configuration metadata
\State \Return $\Delta_s$
\end{algorithmic}
\end{algorithm}
% Both AdamW optimizers have weight_decay=0. The second stage uses
% readout_steps + retrieval_steps = 32 + 32 = 64 updates with the same
% retrieval-aligned objective, not two successive readout objectives.
% LoRA uses alpha=64 in the final eight layers (q,k,v,o,gate,up,down).


==> figures/figure1_pss_rag_pipeline.tex <==
\begin{tikzpicture}[
    x=1cm,y=1cm,
    panel/.style={draw=black!18, line width=.65pt, rounded corners=7pt},
    flow/.style={draw=black!55, rounded corners=2.5pt, align=center,
        minimum height=6.5mm, inner xsep=3pt, font=\tiny},
    input/.style={flow, fill=white},
    baseline/.style={flow, fill=mutedgray},
    pssbox/.style={flow, fill=pssyellow, draw=black!60},
    evidence/.style={flow, fill=raggreen, draw=black!55},
    output/.style={flow, fill=stateblue, draw=black!55},
    failure/.style={flow, fill=failred, draw=black!55},
    arrow/.style={-{Latex[length=1.7mm]}, line width=.65pt, draw=black!78},
    offline/.style={-{Latex[length=1.5mm]}, line width=.55pt,
        densely dashed, draw=black!62},
    lane/.style={font=\bfseries\tiny, align=left},
    title/.style={font=\bfseries\scriptsize, align=center},
    note/.style={font=\tiny, align=center, text=black!72},
    card/.style={draw=black!28, fill=white, rounded corners=4pt,
        text width=3.25cm, minimum height=1.18cm, align=left,
        inner sep=5pt, font=\scriptsize},
    badge/.style={circle, fill=guardgold, draw=black!20, inner sep=1.5pt,
        font=\bfseries\tiny}
]

% ------------------------------------------------------------------
% (a) Inputs and the retrieval bottleneck.
% ------------------------------------------------------------------
\path[panel, fill=mutedgray!28] (-.15,.20) rectangle (4.15,6.85);
\node[title] at (2.0,6.48) {Session input and retrieval gap};

\node[input, minimum width=3.35cm, minimum height=1.05cm] (history)
    at (2.0,5.32) {\textbf{Session history $H_s$}\\
    Orion project $\rightarrow$ checkpoint v5 $\rightarrow$ \textbf{v7}\\
    data source, constraints, and revisions};

\node[input, minimum width=3.35cm, minimum height=.86cm] (query)
    at (2.0,3.75) {\textbf{Current query $q$}\\
    ``Use the previous configuration.''};

\node[baseline, minimum width=3.05cm] (rawterms)
    at (2.0,2.43) {Raw search terms\\use $\cdot$ previous $\cdot$ configuration};
\node[failure, minimum width=3.35cm, minimum height=.88cm] (rawmiss)
    at (2.0,1.10) {\textbf{Standard RAG failure}\\
    Orion and v7 are absent $\Rightarrow$ partial / wrong evidence};
\draw[arrow] (query) -- (rawterms);
\draw[arrow] (rawterms) -- (rawmiss);
\node[note, text=black!58] at (2.0,3.14)
    {needed terms remain only in $H_s$};

\node[badge] at (.22,6.48) {a};

% ------------------------------------------------------------------
% (b) Aligned RAG pipelines.
% ------------------------------------------------------------------
\path[panel, fill=white] (4.45,.20) rectangle (13.85,6.85);
\node[title] at (9.15,6.48) {Where PSS changes the RAG pipeline};

% Standard RAG lane.
\node[lane, anchor=east] at (5.35,5.32) {Standard\\RAG};
\node[input, minimum width=.82cm] (sin) at (6.05,5.32) {$q$};
\node[baseline, minimum width=1.10cm] (sret) at (7.42,5.32) {Retriever};
\node[failure, minimum width=1.30cm] (sevi) at (8.98,5.32)
    {partial\\evidence};
\node[baseline, minimum width=1.08cm] (sgen) at (10.47,5.32) {Base LM};
\node[failure, minimum width=1.55cm] (sout) at (12.25,5.32)
    {incomplete /\\wrong answer};
\draw[arrow] (sin) -- (sret);
\draw[arrow] (sret) -- (sevi);
\draw[arrow] (sevi) -- (sgen);
\draw[arrow] (sgen) -- (sout);

% Full-history RAG lane.
\node[lane, anchor=east] at (5.35,3.80) {Full-history\\RAG};
\node[input, minimum width=1.02cm] (fin) at (6.05,3.80) {$[H_s;q]$};
\node[baseline, minimum width=1.18cm] (frew) at (7.45,3.80)
    {history\\rewrite};
\node[baseline, minimum width=1.08cm] (fret) at (8.86,3.80) {Retriever};
\node[evidence, minimum width=1.18cm] (fevi) at (10.28,3.80)
    {source\\evidence};
\node[baseline, minimum width=1.02cm] (fgen) at (11.64,3.80) {Base LM};
\node[output, minimum width=1.20cm] (fout) at (13.00,3.80)
    {grounded\\answer};
\draw[arrow] (fin) -- (frew);
\draw[arrow] (frew) -- (fret);
\draw[arrow] (fret) -- (fevi);
\draw[arrow] (fevi) -- (fgen);
\draw[arrow] (fgen) -- (fout);
\node[note, text=black!58] at (7.43,3.26) {replays long history online};

% Highlighted PSS-RAG lane and offline writer.
\path[draw=guardgold!85!black, fill=pssyellow!34, rounded corners=5pt,
    line width=.7pt] (4.62,.52) rectangle (13.67,2.92);
\node[lane, anchor=east] at (5.35,1.35) {\textbf{PSS-RAG}\\\textit{ours}};

\node[input, minimum width=.78cm] (phist) at (5.98,2.38) {$H_s$};
\node[pssbox, minimum width=1.18cm] (writer) at (7.38,2.38)
    {offline\\writer};
\node[pssbox, minimum width=1.12cm] (state) at (8.82,2.38)
    {$\Delta_s$\\LoRA state};
\draw[offline] (phist) -- node[above,note]{write once} (writer);
\draw[offline] (writer) -- (state);
\node[note, anchor=west] at (9.52,2.38)
    {fixed shape; session-specific\\24--44 MiB; answer-free objective};

\node[input, minimum width=.78cm] (pin) at (6.02,1.35) {$q$};
\node[pssbox, minimum width=1.38cm] (clue) at (7.58,1.35)
    {intent clue\\$\tilde q_s$};
\node[baseline, minimum width=1.05cm] (pret) at (9.08,1.35) {Retriever};
\node[evidence, minimum width=1.20cm] (pevi) at (10.50,1.35)
    {auditable\\evidence};
\node[baseline, minimum width=1.00cm] (pgen) at (11.88,1.35) {Base LM};
\node[output, minimum width=1.18cm] (pout) at (13.02,1.35)
    {grounded\\answer};
\draw[arrow] (pin) -- (clue);
\draw[offline] (state.south) |- (clue.north);
\draw[arrow] (clue) -- (pret);
\draw[arrow] (pret) -- (pevi);
\draw[arrow] (pevi) -- (pgen);
\draw[arrow] (pgen) -- (pout);
\node[note, text=black!65] at (11.22,.78)
    {unload $\Delta_s$ before generation};

\node[badge] at (4.82,6.48) {b};

% ------------------------------------------------------------------
% (c) Observable outputs and evidence boundary.
% ------------------------------------------------------------------
\path[panel, fill=stateblue!25] (14.15,.20) rectangle (18.35,6.85);
\node[title] at (16.25,6.48) {Observable outputs};

\node[card] (outone) at (16.25,5.25) {\textbf{\hspace{4mm}1. Retrieval intent}\\
    \textit{``Orion v7 configuration''}\\
    Compact clue; not a final answer.};
\node[badge] at (14.62,5.58) {1};

\node[card] (outtwo) at (16.25,3.55) {\textbf{\hspace{4mm}2. Retrieved evidence}\\
    Top-$k$ source chunks contain the exact checkpoint, version, and constraints.};
\node[badge] at (14.62,3.88) {2};

\node[card] (outthree) at (16.25,1.75) {\textbf{\hspace{4mm}3. Grounded response}\\
    Frozen base LM answers from inspectable evidence after the session state is unloaded.};
\node[badge] at (14.62,2.08) {3};

\draw[arrow] (outone) -- (outtwo);
\draw[arrow] (outtwo) -- (outthree);
\node[note, text width=3.65cm] at (16.25,.66)
    {Causal checks: correct state $>$ wrong / shuffled / zero;\\
    answer-stage keep $\approx$ unload.};
\node[badge] at (14.52,6.48) {c};

\end{tikzpicture}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

